Typing a Core Binary Field Arithmetic in a Light Logic

We design a library for binary field arithmetic and we supply a core API which is completely developed in DLAL, extended with a fix point formula. Since DLAL is a restriction of linear logic where only functional programs with polynomial evaluation cost can be typed, we obtain the core of a functional programming setting for binary field arithmetic with built-in polynomial complexity.

==> API-figure.tex <==
\begin{figure}%Type assignment API
\fbox{
\begin{minipage}{.97\textwidth}
{\small
%% line 0
\[
\infer[\bfLstE]
      {\bfJudg{}{\wNil}{\bfType}}
      {}
\qquad\qquad
\infer[\bfLst]
      {\bfJudg{}{\wExt{\Seq{\bBit{0}}{\bBit{n-1}}}}{\bfType}}
      {}
\qquad\qquad
\infer[\bfO]
      {\bfJudg{}{o}{A}}
      { \vdash_{\TFA} o \!\hasType\! A
        &
        o\in\bfOp}
\]
%% line 1
\[
\infer[\bfAx]
      {\bfJudg{\bfCntxL,\bfCntxB{x}{A}}{x}{A}}
      {}
\qquad\qquad
\qquad\qquad
\infer[\bfPL]
        {
          \bfJudg{}
                 {\lcPL{}{M}}
                 {\lPar A\lImpl\lPar B}
        }{
          \bfJudg{}
                 {M}{A\lImpl B}
        }
\]
%% line 2
\[
\infer[\bfLII]
        {
          \bfJudg{\bfCntxL}{\lcF{x}{M}}{A\lImpl B}
        }{
          \bfJudg{\bfCntxL,\bfCntxB{x}{A}}{M}{B}
        }
\qquad\qquad
\infer[\bfLIE]
        {
           \bfJudg{\bfCntxL,\bfCntxL'}{\lcA{M}{N}}{B}
        }{
          \bfJudg{\bfCntxL}{M}{A\lImpl B}
          &
          \bfJudg{\bfCntxL'}{N}{A}
        }
\]
%% line 3
\[
\infer[\bfLIIp]
        {
          \bfJudg{\bfCntxL}
                 {\lcTD{\Seq{x_1}{x_n}}{M}}
                 {\pTypeC{A_1}{\Seq{\lTime}{\lTime}}{A_n}\lImpl B}
        }{
          \bfJudg{\bfCntxL
                 ,\Seq{\bfCntxB{x_1}{A_1}}
                      {\bfCntxB{x_n}{A_n}}
                 }
                 {M}{B}
        }
\qquad
\infer[\bfTup]
        {
           \bfJudg{\Seq{\bfCntxL_1}{\bfCntxL_n}}
                  {\lcTC{\Seq{M_1}{M_n}}}
                  {\pTypeC{A_1}{\Seq{\lTime}{\lTime}}{A_n}}
        }{
          \bfJudg{\bfCntxL_1}
                 {M_1}
                 {A_1}
          &
          \ldots
          &
          \bfJudg{\bfCntxL_n}
                 {M_n}
                 {A_n}
        }
\]
}%\small
\end{minipage}
}%\fbox
\caption{Type assignment $\bfAPI$}
\label{fig:Type assignment bfAPI}
\end{figure}
 

